Convergence and Trade-Offs in Riemannian Gradient Descent and Riemannian Proximal Point

In this work, we analyze two of the most fundamental algorithms in geodesically convex optimization: Riemannian gradient descent and (possibly inexact) Riemannian proximal point. We quantify their rates of convergence and produce different variants with several trade-offs. Crucially, we show the iterates naturally stay in a ball around an optimizer, of radius depending on the initial distance and, in some cases, on the curvature. In contrast, except for limited cases, previous works bounded the maximum distance between iterates and an optimizer only by assumption, leading to incomplete analyses and unquantified rates. We also provide an implementable inexact proximal point algorithm yielding new results on minmax problems, and we prove several new useful properties of Riemannian proximal methods: they work when positive curvature is present, the proximal operator does not move points away from any optimizer, and we quantify the smoothness of its induced Moreau envelope. Further, we explore beyond our theory with empirical tests.

==> definitions.tex <==
\usepackage{xparse}
\usepackage{xargs}

\makeatletter 
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} 
\makeatother


\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{(\cref{#1})\newtarget{proof:#1}\ }

\usepackage[bb=boondox]{mathalpha} 
\newcommand{\zeros}{\mathbb{0}} 
\newcommand\Hess{\operatorname{Hess}}


\newcommand{\innp}[1]{\langle #1 \rangle}
\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigoast}[1]{O^\ast( #1 )}
\newcommand{\bigoastl}[1]{O^\ast\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}

\DeclarePairedDelimiter\card{\lvert}{\rvert}    
\newcommand{\pa}[1]{\left( #1\right)} 
\newcommand{\norm}[1]{\| #1 \|} 
\newcommand{\norml}[1]{\left\| #1 \right\|} 
\newcommand{\abs}[1]{\lvert #1 \rvert} 
\DeclarePairedDelimiter\cor{\lbrack}{\rbrack}   
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}    

\newcommand*\circledaux[1]{\tikz[baseline=(char.base)]{
\node[shape=circle,draw,inner sep=0.8pt] (char) {#1};}}

\NewDocumentCommand{\circled}{m o }{%
\IfNoValueTF{#2}{\circledaux{#1}}{\stackrel{\circledaux{#1}}{#2}}%
}

\DeclareMathOperator{\supp}{supp}                       
\DeclareMathOperator*{\diag}{diag}                      
\renewcommand*{\Im}{\mathrm{Im}}                        
\newcommand*\dif{\mathrm{d}}                            
\newcommand*\Id{\mathrm{Id}}                            
\newcommand\conn{\nabla}                                
\newcommand*\tensor{\otimes}                            
\newcommand{\defi}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\defiin}{\stackrel{\mathrm{\scriptscriptstyle def}}{\in}}
\newcommand*\iso{\cong}                                 
\newcommand*\fn{\operatorname}                          
\newcommand{\code}{\texttt}                             
\newcommand\deriv[1]{\frac{\mathrm{d}}{\mathrm{d}#1}}   

\renewcommand*\C{\mathbb{C}}                              
\renewcommand*\R{\mathbb{R}}                              
\newcommand*\Z{\mathbb{Z}}                                
\newcommand*\mean[1]{\overline{#1}}                       

\let\epsilon\varepsilon



\newcommand\trans[1]{#1^\intercal}                          
\DeclareMathOperator\tr{tr}                                 
\newcommand\dual[1]{#1^\ast}                                
\newcommand\faprox{f_{\delta, L}}                           
\newcommand\gaprox{g_{\delta, L}}                           
\newcommand\Mani{\mathcal{M}}                               
\renewcommand\S{\mathbb{S}}                                 
\DeclareMathOperator\gradmani{grad}                         
\newcommand\gradexp{\tilde{\grad}}                          
\DeclareMathOperator\ad{ad}                                 
\DeclareMathOperator\Ad{Ad}                                 
\newcommand\g{\mathfrak{g}}                                 
\DeclareMathOperator{\End}{End}                             
\newcommand\adj[1]{#1^\ast}                                 
\DeclareMathOperator{\normal}{\mathcal{N}}                  
\DeclareMathOperator{\unif}{\mathcal{U}}                    
\newcommand\I{\mathrm{I}}                                   


\newcommand{\Var}[1]{\text{Var}\left[#1\right]} 
\newcommand{\Cov}[1]{\text{Cov}\left[#1\right]} 
\renewcommand{\P}[1]{\mathbb{P}\left[#1\right]} 
\newcommand{\Vart}{\text{Var}} 
\renewcommand{\E}[1]{\mathbb{E}\left[ #1 \right]} 
\newcommand{\dirich}[1]{\mathcal{E}\left( #1 \right)} 
\newcommand{\grad}{\nabla} 
\newcommand{\ones}{\mathds{1}}                           
\newcommand{\varl}{\operatorname{left}} 
\newcommand{\varr}{\operatorname{right}} 


\usepackage{pifont} 
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\yesmark}{{\color{green} \cmark}}
\newcommand{\nomark}{{\color{red} \xmark}}


\DeclareMathOperator*{\argmax}{arg\,max}                
\DeclareMathOperator*{\argmin}{arg\,min}                


\let\oldmu\mu
\renewcommand\mu{\newlink{def:strong_g_convexity_of_F}{\oldmu}}

\newcommandx*{\Lips}[1][1=, usedefault]{\newlink{def:Lipschitz_constant}{L_{\operatorname{p}}^{#1}}}
\let\strikedL\L
\renewcommand{\L}{\newlink{def:riemannian_smoothness_of_F}{L}} 




\newcommand{\RGD}{\newlink{def:acronym_riemannian_gradient_descent}{RGD}}
\newcommand{\RGDA}{\newlink{def:acronym_riemannian_gradient_descent_ascent}{RGDA}}
\newcommand{\CRGD}{\newlink{def:acronym_composite_riemannian_gradient_descent}{CRGD}}
\newcommand{\PRGD}{\newlink{def:acronym_metric_projected_riemannian_gradient_descent}{PRGD}}
\newcommand{\RPPA}{\newlink{def:acronym_riemannian_proximal_point_algorithm}{RPPA}}
\newcommand{\RIPPA}{\newlink{def:acronym_riemannian_inexact_proximal_point_algorithm}{RIPPA}}
\newcommand{\RCEGmin}{\newlink{def:acronym_rceg_min}{RCEG-min}}
\newcommand{\RCEG}{\newlink{def:acronym_rceg}{RCEG}}

\renewcommand\M{\mathcal{M}}
\renewcommand\H{\mathcal{H}}
\newcommand\NN{\newlink{def:N_open_set_in_manifold}{\mathcal{N}}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Xt}{\mathcal{X}_{t}}

\newcommandx*{\Rmax}[1][1=, usedefault]{\newlink{def:max_distance_to_x_ast}{R_{\max}^{#1}}}
\renewcommand{\R}{\newlink{def:initial_distance}{R}}
\newcommandx*\kmin[1][1=, usedefault]{\newlink{def:minimum_sectional_curvature}{\kappa_{\min}^{#1}}}
\newcommandx*\kmax[1][1=, usedefault]{\newlink{def:maximum_sectional_curvature}{\kappa_{\max}^{#1}}}
\newcommand\Mmin{\mathcal{M}_{\operatorname{LB}}}
\newcommand\Riemmin{\newlink{def:M_manifold_with_lower_bounded_curv}{\mathcal{R}_{\operatorname{LB}}}}
\newcommand\Riem{\newlink{def:M_manifold_with_lower_bounded_curv}{\mathcal{R}_{\operatorname{LUB}}}}

\newcommand{\dist}{\newlink{def:distance}{d}}

\newcommandx*\prox[2][1=f, 2=\eta, usedefault]{\newlink{def:prox}{\operatorname{prox}_{#2#1}}}

\newcommandx*\smc[1][1=\X, usedefault]{\newlink{def:smooth_convex_class}{\mathcal{F}_{\L}(#1)}}
\newcommandx*\smsc[3][1=\X, 2=\L, 3=\mu, usedefault]{\newlink{def:smooth_strongly_convex_class}{\mathcal{F}_{#3, #2}(#1)}}
\newcommandx*\nsmc[1][1=\X, usedefault]{\newlink{def:non_smooth_convex_class}{\mathcal{F}_{\Lips}(#1)}}
\newcommandx*\proxc[1][1=\M, usedefault]{\newlink{def:proper_lsc_convex_class}{\mathcal{F}(#1)}}
\newcommandx*\proxsp[1][1=\X, usedefault]{\newlink{def:convex_concave_class}{\mathcal{F}_{SP}(#1)}}

\newcommand{\diam}{\operatorname{diam}}
 
\newcommand\ball{\newlink{def:closed_ball}{\bar{B}}}

\newcommand\xast{\newlink{def:optimizer}{x^\ast}}

\newcommand\expon[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Exp}_{#1}}}
\newcommand\exponinv[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Log}_{#1}}} 

\newcommandx*\proj[1][1=\X, usedefault]{\newlink{def:projection_operator}{\mathcal{P}_{#1}}}

\newcommand\inj{\operatorname{inj}}

\newcommand{\Y}{\mathcal{Y}}
\newcommand{\XX}{\mathcal{X}} 

\newcommand\N{\mathcal{N}}

\newcommand\indicator[1]{\newlink{def:indicator_function}{I_{#1}}}


\renewcommand\d{\mathrm{d}}

\newcommand\Tansp[1]{\newlink{def:tangent_space}{T_{#1}}}

\let\oldGamma\Gamma
\renewcommand{\Gamma}[2]{\newlink{def:parallel_transport}{\oldGamma_{#1}^{#2}}}

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}



\let\oldzeta\zeta
\renewcommand\zeta{\newlink{def:zeta_geometric_constant}{\oldzeta}}

\let\olddelta\delta
\renewcommand\delta{\newlink{def:delta_geometric_constant}{\olddelta}}

\newcommand\xinit{\newlink{def:initial_point}{x_0}}

\newcommand\yinit{y_0}
\newcommand\yast{y^\ast}
\newcommand\zinit{z_0}
\newcommand\zast{z^\ast}

\newcommand{\rt}{r_{t}}
\newcommand{\rtp}{r_{t+1}}
\newcommand{\rtx}{r_{t}^x}
\newcommand{\rtpx}{r_{t+1}^x}
\newcommand{\rty}{r_{t}^y}
\newcommand{\rtpy}{r_{t+1}^y}

